KAT-V1: Kwai-AutoThink Technical Report

We present Kwaipilot-AutoThink (KAT), an open-source 40B large language model developed to address the overthinking problem in reasoning-intensive tasks, where an automatic thinking training paradigm is proposed to dynamically switch between reasoning and non-reasoning modes based on task complexity. Specifically, first, we construct the dual-regime dataset based on a novel tagging pipeline and a multi-agent synthesis strategy, and then we apply Multi-Token Prediction (MTP)-enhanced knowledge distillation, enabling efficient and fine-grained reasoning transfer with minimal pretraining cost. Besides, we implement a cold-start initialization strategy that introduces mode-selection priors using majority-vote signals and intent-aware prompting. Finally, we propose Step-SRPO, a reinforcement learning algorithm that incorporates intermediate supervision into the GRPO framework, offering structured guidance over both reasoning-mode selection and response accuracy. Extensive experiments across multiple benchmarks demonstrate that KAT consistently matches or even outperforms current state-of-the-art models, including DeepSeek-R1-0528 and Qwen3-235B-A22B, across a wide range of reasoning-intensive tasks while reducing token usage. Notably, KAT outperforms all open-source models and even surpasses o3-mini on the leakage-controlled LiveCodeBench Pro. Beyond academic evaluation, KAT has been successfully deployed in Kwaipilot (i.e., Kuaishou's internal coding assistant), where it improves real-world development workflows with high accuracy, efficiency, and controllable reasoning behaviors. Moreover, we are actively training a 200B Mixture-of-Experts (MoE) model with 40B active parameters, and early results already show significant gains, further demonstrating the scalability of the AutoThink paradigm.

==> sections/analysis-on-xxx.tex <==
\section{Results}

To evaluate the effectiveness of Kwaipilot-AutoThink (KAT), we compared our model with several leading open-source state-of-the-art (SOTA) models, including LLaMA-4-Scout, LLaMA-4-Maverick, Qwen3-32B, Qwen3-235B-A22B, DeepSeek-V3, and DeepSeek-R1-0528 across a variety of benchmarks. As shown in Table~\ref{tab:main-comparison}, KAT consistently matches or outperforms these models in terms of accuracy across tasks in general reasoning, math and text reasoning, as well as agent and coding tasks.

\begin{table*}[htbp]
\centering
\caption{Comparison of KAT and leading SOTA models across diverse benchmark tasks-new.}
\label{tab:main-comparison}

% ========= 上半部分，前4个模型 ==========
\resizebox{\textwidth}{!}{
\begin{tabular}{l
                cc
                cc
                cc
                cc
                }
\toprule
&
\multicolumn{2}{c}{\textbf{KAT-V1-40B}} &
\multicolumn{2}{c}{\textbf{KAT-200B}} &
\multicolumn{2}{c}{\textbf{DeepSeek-R1-0528}} &
\multicolumn{2}{c}{\textbf{Qwen3-235B-A22B}} \\
\midrule
Architecture         & \multicolumn{2}{c}{Dense} & \multicolumn{2}{c}{MoE} & \multicolumn{2}{c}{MoE} & \multicolumn{2}{c}{MoE} \\
\# Total Params      & \multicolumn{2}{c}{40B} & \multicolumn{2}{c}{200B} & \multicolumn{2}{c}{671B} & \multicolumn{2}{c}{235B} \\
\# Activated Params  & \multicolumn{2}{c}{40B} & \multicolumn{2}{c}{40B}  & \multicolumn{2}{c}{37B}  & \multicolumn{2}{c}{22B}  \\
\midrule
& Score & Token Usage & Score & Token Usage & Score & Token Usage & Score & Token Usage \\
\midrule
\multicolumn{9}{c}{\textit{General Tasks}} \\
\cmidrule(lr){1-9}
GPQA-Diamond\cite{rein2024gpqa-Diamond}  & \underline{75.1} & \textcolor{lightgray}{6604}   & \textbf{78.2} & \textcolor{lightgray}{10386}  & \fbox{81.0} & \textcolor{lightgray}{8272} & 71.1 & \textcolor{lightgray}{10591}    \\
MMLU-Pro\cite{wang2024mmlu-pro}          & 77.8 & \textcolor{lightgray}{2316}   & \fbox{82.3} & \textcolor{lightgray}{3726}   & \textbf{81.9} & \textcolor{lightgray}{3538} & 80.8 & \textcolor{lightgray}{3005}   \\
DROP\cite{Dua2019DROP}                   & 91.2 & \textcolor{lightgray}{613}    & \underline{91.6} & \textcolor{lightgray}{1125}   & \fbox{92.2} & \textcolor{lightgray}{1896}   & \textbf{91.9} & \textcolor{lightgray}{1058}  \\
WildBench\cite{lin2024wildbench}         & 8.73 & \textcolor{lightgray}{12817}  & \textbf{8.77} & \textcolor{lightgray}{15247}  & \fbox{8.80} & \textcolor{lightgray}{14502}  & 8.72 & \textcolor{lightgray}{18057} \\
\midrule
\multicolumn{9}{c}{\textit{Math \& Text Reasoning}} \\
\cmidrule(lr){1-9}
MATH500\cite{huggingface-math500}        & \underline{97.4} & \textcolor{lightgray}{4302}   & \textbf{97.6} & \textcolor{lightgray}{7351}   & 97.3 & \textcolor{lightgray}{7135}   & \fbox{98.0} & \textcolor{lightgray}{7161}  \\
AIME2024\cite{huggingface-aime2024}      & \textbf{93.3} & \textcolor{lightgray}{15716}  & \fbox{96.3} & \textcolor{lightgray}{19635}  & \underline{91.4} & \textcolor{lightgray}{20523}  & 85.7 & \textcolor{lightgray}{17274} \\
AIME2025\cite{huggingface-aime2025}      & \textbf{88.1} & \textcolor{lightgray}{19132}  & \fbox{90.4} & \textcolor{lightgray}{27410}  & \underline{87.5} & \textcolor{lightgray}{24648}  & 81.5 & \textcolor{lightgray}{20460} \\
AutoLogi\cite{zhu2025autologi}           & 81.2 & \textcolor{lightgray}{3316}   & \underline{84.9} & \textcolor{lightgray}{8328}   & 84.3 & \textcolor{lightgray}{5898}   & \fbox{89.0} & \textcolor{lightgray}{8770}  \\
\midrule
\multicolumn{9}{c}{\textit{Agent \& Coding Tasks}} \\
\cmidrule(lr){1-9}
HumanEval\cite{chen2021openai-humaneval} & \underline{95.1} & \textcolor{lightgray}{832}    & \fbox{98.2} & \textcolor{lightgray}{1339}   & \textbf{97.0} & \textcolor{lightgray}{524}    & 30.5 & \textcolor{lightgray}{4731}  \\
MBPP\cite{austin2021mbpp}                & \underline{90.8} & \textcolor{lightgray}{2007}   & \textbf{93.2} & \textcolor{lightgray}{2976}   & \fbox{96.2} & \textcolor{lightgray}{3938}   & 65.4 & \textcolor{lightgray}{7420}  \\
EvalPlus\cite{evalplus-1,evalplus-2}     & 76.0 & \textcolor{lightgray}{1339}   & \fbox{80.4} & \textcolor{lightgray}{2441}   & \textbf{79.2} & \textcolor{lightgray}{3211}   & 77.6 & \textcolor{lightgray}{5434}  \\
LiveCodeBench\cite{jain2024livecodebench}& \textbf{74.2} & \textcolor{lightgray}{13087}  & \fbox{77.1} & \textcolor{lightgray}{18362}  & \underline{73.3} & \textcolor{lightgray}{17956}  & 59.1 & \textcolor{lightgray}{21049}   \\
BFCL-V3-Multiturn\cite{patil2025bfcl-v3} & 39.0 & \textcolor{lightgray}{2418}    & \textbf{41.6} & \textcolor{lightgray}{3393}    & 38.9 & \textcolor{lightgray}{12286}   & \underline{40.1} & \textcolor{lightgray}{4799}    \\
\bottomrule
\end{tabular}
}

\vspace{2mm}

% ========= 下半部分，后4个模型 ==========
\resizebox{\textwidth}{!}{
\begin{tabular}{l
                cc
                cc
                cc
                cc
                }
\toprule
&
\multicolumn{2}{c}{\textbf{DeepSeek-V3}} &
\multicolumn{2}{c}{\textbf{LLaMA-4-Maverick}} &
\multicolumn{2}{c}{\textbf{LLaMA-4-Scout}} &
\multicolumn{2}{c}{\textbf{Qwen3-32B}} \\
\midrule
Architecture         & \multicolumn{2}{c}{MoE} & \multicolumn{2}{c}{MoE} & \multicolumn{2}{c}{MoE} & \multicolumn{2}{c}{Dense} \\
\# Total Params      & \multicolumn{2}{c}{671B} & \multicolumn{2}{c}{400B} & \multicolumn{2}{c}{109B} & \multicolumn{2}{c}{32B} \\
\# Activated Params  & \multicolumn{2}{c}{37B}  & \multicolumn{2}{c}{17B}  & \multicolumn{2}{c}{17B}  & \multicolumn{2}{c}{32B}  \\
\midrule
& Score & Token Usage & Score & Token Usage & Score & Token Usage & Score & Token Usage \\
\midrule
\multicolumn{9}{c}{\textit{General Tasks}} \\
\cmidrule(lr){1-9}
GPQA-Diamond  & 68.4 & \textcolor{lightgray}{1559} & 69.8 & \textcolor{lightgray}{1014} & 57.2 & \textcolor{lightgray}{899} & 68.4 & \textcolor{lightgray}{5477}  \\
MMLU-Pro     & \underline{81.2} & \textcolor{lightgray}{708} & 80.5 & \textcolor{lightgray}{567} & 74.3 & \textcolor{lightgray}{466} & 76.2 & \textcolor{lightgray}{1776} \\
DROP          & 90.5 & \textcolor{lightgray}{162}  & 90.7 & \textcolor{lightgray}{170} & 89.2 & \textcolor{lightgray}{156} & 91.1 & \textcolor{lightgray}{451}   \\
WildBench     & \underline{8.74} & \textcolor{lightgray}{4397} & 8.29 & \textcolor{lightgray}{3877} & 8.21 & \textcolor{lightgray}{4399} & 8.56 & \textcolor{lightgray}{16566}  \\
\midrule
\multicolumn{9}{c}{\textit{Math \& Text Reasoning}} \\
\cmidrule(lr){1-9}
MATH500       & 94.0 & \textcolor{lightgray}{1453} & 90.6 & \textcolor{lightgray}{709} & 82.6 & \textcolor{lightgray}{684} & 97.2 & \textcolor{lightgray}{4894}  \\
AIME2024      & 59.4 & \textcolor{lightgray}{3972} & 38.5 & \textcolor{lightgray}{1378} & 28.6 & \textcolor{lightgray}{1256} & 81.4 & \textcolor{lightgray}{12999}  \\
AIME2025      & 44.2 & \textcolor{lightgray}{3980} & 15.9 & \textcolor{lightgray}{1376} & 10.0 & \textcolor{lightgray}{1209} & 72.9 & \textcolor{lightgray}{15436}  \\
AutoLogi      & 76.1 & \textcolor{lightgray}{1809} & 75.2 & \textcolor{lightgray}{904} & 56.8 & \textcolor{lightgray}{788} & \textbf{87.3} & \textcolor{lightgray}{4286}  \\
\midrule
\multicolumn{9}{c}{\textit{Agent \& Coding Tasks}} \\
\cmidrule(lr){1-9}
HumanEval     & 93.3 & \textcolor{lightgray}{175}  & 88.4 & \textcolor{lightgray}{78} & 83.5 & \textcolor{lightgray}{200} & 90.2 & \textcolor{lightgray}{2804}   \\
MBPP          & 83.6 & \textcolor{lightgray}{758}  & 81.0 & \textcolor{lightgray}{246} & 72.0 & \textcolor{lightgray}{489} & 74.6 & \textcolor{lightgray}{4229}  \\
EvalPlus      & \underline{78.9} & \textcolor{lightgray}{320}  & 75.8 & \textcolor{lightgray}{202} & 67.7 & \textcolor{lightgray}{386} & 72.1 & \textcolor{lightgray}{3125}  \\
LiveCodeBench & 44.7 & \textcolor{lightgray}{2094} & 34.1 & \textcolor{lightgray}{792} & 30.2 & \textcolor{lightgray}{927} & 61.5 & \textcolor{lightgray}{13616}  \\
BFCL-V3-Multiturn & 29.9 & \textcolor{lightgray}{701}   & 16.4 & \textcolor{lightgray}{406} & 1.9 & \textcolor{lightgray}{444} & \fbox{43.1} & \textcolor{lightgray}{4807}  \\
\bottomrule
\end{tabular}
}
\end{table*}

In addition to competitive accuracy, KAT demonstrates significant improvements in token efficiency. For example, across various benchmarks, the average token savings range from 11.6 to 89.9 percent. Notably, for the 40B model, the average token usage is approximately 72.7 percent of that used by DeepSeek-R1-0528, showing substantial efficiency gains.
These improvements are enabled by KAT's dynamic reasoning control, which selectively activates reasoning only when necessary, significantly reducing token usage in simpler queries. The model adapts its reasoning depth based on task complexity, resulting in fewer tokens consumed without sacrificing response quality.

In summary, Kwaipilot-AutoThink offers both high performance and enhanced efficiency, driven by a strong reasoning control strategy and an adaptive approach to token usage. This makes KAT a resource-efficient solution for real-world applications, as evidenced by its integration into Kwaipilot, Kuaishou's internal coding assistant.

==> sections/experiments.tex <==
\section{Experiments}

\subsection{Evaluation and Performance}
We conducted thorough evaluations of Step-SRPO across established benchmarks spanning mathematical reasoning, advanced QA, coding tasks, and instruction-following scenarios. Consistent hyperparameters were utilized throughout experiments: a learning rate of $1 \times 10^{-6}$, a global batch size of 64 queries per policy update, and 32 generated trajectories per query, yielding approximately 2{,}048 samples per update. This configuration ensured sufficient diversity and stability for robust AutoThink reinforcement and performance enhancement.

All results are reported as accuracy or pass rate (\%). The baseline model is a supervised fine-tuned (SFT) checkpoint, and Step-SRPO denotes the model after 10 steps of reinforcement learning on top of this SFT base.


\begin{table*}[ht]
\centering
\caption{
\textbf{Comparison among models.}
The highest and second-best scores are shown in \textbf{bold} and \uline{underline}, respectively.
}
\label{tab:main-comparison}
\resizebox{\textwidth}{!}{
\begin{tabular}{l
                cc
                cc
                cc
                cc
                cc}
\toprule
& 
\multicolumn{2}{c}{\textbf{Qwen2.5-72B Base}} &
\multicolumn{2}{c}{\textbf{Qwen2.5-Plus Base}} &
\multicolumn{2}{c}{\textbf{Llama-4-Maverick Base}} &
\multicolumn{2}{c}{\textbf{DeepSeek-V3 Base}} &
\multicolumn{2}{c}{\textbf{Qwen3-235B-A22B Base}} 
\\
& Score & Token Usage & Score & Token Usage & Score & Token Usage & Score & Token Usage & Score & Token Usage
\\
\midrule
Architecture & Dense & & MoE & & MoE & & MoE & & MoE & \\
\# Total Params & 72B & & 271B & & 402B & & 671B & & 235B & \\
\# Activated Params & 72B & & 37B & & 17B & & 37B & & 22B & \\
\midrule
\multicolumn{11}{c}{\textit{General Tasks}} \\
\cmidrule(lr){1-11}
MMLU        & 86.06  & 1200  & 85.02 & 1100  & 85.16 & 1050  & \uline{87.19} & 1250  & \textbf{87.81} & 1180 \\
MMLU-Redux  & 83.91  & 800   & 82.69 & 700   & 84.05 & 710   & \uline{86.14} & 810   & \textbf{87.40} & 780  \\
MMLU-Pro    & 58.07  & 1700  & 63.52 & 1850  & \uline{63.91} & 1900  & 59.84 & 1650  & \textbf{68.18} & 1980 \\
SuperGPQA   & 36.20  & 900   & 37.18 & 950   & 40.85 & 890   & \uline{41.53} & 930   & \textbf{44.06} & 980  \\
BBH         & 86.30  & 1400  & 85.60 & 1300  & 83.62 & 1280  & \uline{86.22} & 1320  & \textbf{88.87} & 1340 \\
\midrule
\multicolumn{11}{c}{\textit{Math \& STEM Tasks}} \\
\cmidrule(lr){1-11}
GPQA        & \uline{45.88}  & 600  & 41.92 & 500   & 43.94 & 520   & 41.92 & 610   & \textbf{47.47} & 670  \\
GSM8K       & 91.50  & 1300  & \uline{91.89} & 1220  & 87.72 & 1400  & 87.57 & 1350  & \textbf{94.39} & 1510 \\
MATH        & 62.12  & 2000  & 62.78 & 1900  & \uline{63.32} & 2300  & 62.62 & 1800  & \textbf{71.84} & 2100 \\
\midrule
\multicolumn{11}{c}{\textit{Coding Tasks}} \\
\cmidrule(lr){1-11}
EvalPlus    & 65.93  & 1550  & 61.43 & 1460  & \uline{68.38} & 1590  & 63.75 & 1540  & \textbf{77.60} & 1690 \\
MultiPL-E   & 58.70  & 1050  & 62.16 & 1040  & 57.28 & 1110  & \uline{62.26} & 1130  & \textbf{65.94} & 1250 \\
MBPP        & 76.00  & 1800  & 74.60 & 1720  & \uline{75.40} & 1810  & 74.20 & 1700  & \textbf{81.40} & 1920 \\
CRUX-O      & 66.20  & 1200  & 68.50 & 1250  & \uline{77.00} & 1230  & 76.60 & 1270  & \textbf{79.00} & 1310 \\
\midrule
\multicolumn{11}{c}{\textit{Multilingual Tasks}} \\
\cmidrule(lr){1-11}
MGSM        & 82.40  & 790   & 82.21 & 830   & 79.69 & 810   & \uline{82.68} & 805   & \textbf{83.53} & 830  \\
MMMLU       & 84.40  & 850   & 83.49 & 880   & 83.09 & 870   & \uline{85.88} & 875   & \textbf{86.70} & 900  \\
INCLUDE     & 69.05  & 900   & 66.97 & 910   & \uline{73.47} & 920   & 75.17 & 930   & \textbf{73.46} & 940  \\
\bottomrule
\end{tabular}
}
\end{table*}


\subsubsection{Think-On vs. Think-Off Dynamics During Training}

We logged how often the model chose \texttt{<think\_on>} versus \texttt{<think\_off>} at each step. This shift---visualized in Figure~\ref{fig:step-srpo-gating}---confirms that Step-SRPO not only improves final accuracy but also refines the model's gating behavior, enabling it to skip heavy reasoning when unnecessary.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figutes/thinkOnOffRate.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

\subsection{Token Count Dynamics During Training}
During AutoThink RL training, the average output token count per prediction exhibits a clear downward trend\ref{fig:nothing}. This reduction indicates that the model progressively learns to generate more concise responses, selectively invoking explicit reasoning only when necessary. Such behavior demonstrates the effectiveness of the Step-SRPO reward design in promoting efficient use of chain-of-thought and controlling response length across diverse queries. 

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figutes/avgTokenTrend.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

==> sections/fromDense-to-Sparse.tex <==
\section{From Dense to Sparse: Upcycling of Kwaipilot-AutoThink to 200B MoE}

To further extend the capabilities of Kwaipilot-AutoThink, we have successfully scaled the model from a 40B dense architecture to a 200B Mixture-of-Experts (MoE) model. This new version significantly expands model capacity while maintaining compute efficiency by activating only a small subset of experts per input.

This upscaled 200B model marks a major milestone in the evolution of Kwaipilot-AutoThink, enabling more powerful and controllable reasoning capabilities. We have completed its initial training and will begin integrating it into our internal product, Kwaipilot, to support real-world development workflows with enhanced performance and flexibility.
Preliminary evaluations show that the model delivers strong performance across a wide range of reasoning tasks, as detailed in Table \ref{tab:task-performance-moe}. We also plan to open-source this 200B-parameter, 40B-activated MoE model in the near future, contributing a high-capacity, sparsely activated foundation model to the open LLM community.


\begin{table*}[ht]
\centering
\caption{
\textbf{Benchmark performance of KAT-200B
}
\label{tab:task-performance-moe}
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c c}
\toprule
\textbf{Benchmark} & \multicolumn{2}{c}{\textbf{Kwaipilot--AutoThink--ColdStart: Think--on}} & \multicolumn{2}{c}{\textbf{Kwaipilot--AutoThink--ColdStart: Think--off}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 
 & \textbf{Performance} & \textbf{Token Usage} & \textbf{Performance} & \textbf{Token Usage} \\
\midrule
\multicolumn{5}{c}{\textit{General Tasks}} \\
\cmidrule(lr){1-5}
GPQA--Diamond & 61.1 & 6159 &  &  \\
MMLU--Pro     & 70.8 & 591  &  &  \\
DROP          & 89.2 & 139  &  &  \\
LiveBench     &  &  &  &  \\
\midrule
\multicolumn{5}{c}{\textit{Alignment Tasks}} \\
\cmidrule(lr){1-5}
IFEval        & 79.67 & 380  &  &  \\
Arena--Hard   &  &  &  &  \\
WildBench     &  &  &  &  \\
\midrule
\multicolumn{5}{c}{\textit{Math \& Text Reasoning}} \\
\cmidrule(lr){1-5}
GSM8K         & 93.3  & 144  &  &  \\
MATH500       & 88.4  & 1308 &  &  \\
AIME2024      & 71.25 & 10223 &  &  \\
AIME2025      &  &  &  &  \\
ZebraLogic    &  &  &  &  \\
AutoLogi      &  &  &  &  \\
\midrule
\multicolumn{5}{c}{\textit{Agent \& Coding}} \\
\cmidrule(lr){1-5}
HumanEval     & 91.46 & 179  &  &  \\
MBPP          & 79.8  & 754  &  &  \\
MultiPL--E    &  &  &  &  \\
EvalPlus      &  &  &  &  \\
BigCodeBench  &  &  &  &  \\
CruxEval      &  &  &  &  \\
LiveCodeBench & 54.8  & 8250 &  &  \\
BFCL v3       &  &  &  &  \\
\bottomrule
\end{tabular}
}
\end{table*}
